Meta-Learning for Airflow Simulations with Graph Neural Networks

The field of numerical simulation is of significant importance for the design and management of real-world systems, with partial differential equations (PDEs) being a commonly used mathematical modeling tool. However, solving PDEs remains still a challenge, as commonly used traditional numerical solvers often require high computational costs. As a result, data-driven methods leveraging machine learning (more particularly Deep Learning) algorithms have been increasingly proposed to learn models that can predict solutions to complex PDEs, such as those arising in computational fluid dynamics (CFD). However, these methods are known to suffer from poor generalization performance on out-of-distribution (OoD) samples, highlighting the need for more efficient approaches. To this end, we present a meta-learning approach to enhance the performance of learned models on OoD samples. Specifically, we set the airflow simulation in CFD over various airfoils as a meta-learning problem, where each set of examples defined on a single airfoil shape is treated as a separate task. Through the use of model-agnostic meta-learning (MAML), we learn a meta-learner capable of adapting to new tasks, i.e., previously unseen airfoil shapes, using only a small amount of task-specific data. We experimentally demonstrate the efficiency of the proposed approach for improving the OoD generalization performance of learned models while maintaining efficiency.

==> CFD_Problem.tex <==
\section{Problem Set-Up} % state airfoil design !!! Require designs that are different from the training set.
Analyzing the flow fields around airfoils using the so-called Navier-Stokes PDE to represent the physical system is a classical use case in CFD. The traditional CFD solvers compute the velocity field and the pressure of the flow arounding the airfoil, enabling the understanding and improvement of airfoil properties and designs. 

\subsubsection{CFD Background}
The simplified Reynolds-averaged Navier-Stokes (RANs) equations \cite{reynolds1895iv} are time-averaged equations of motion for fluid flows that are commonly used for airfoil simulations. The system modeled by RANS equations can be expressed as:
\begin{align} \label{eq:RANs}
    \frac{\partial{u_i}}{\partial x_i} = 0 \\
    u_j \frac{\partial{u_i}}{\partial x_j} = \frac{\partial}{\partial x_j} [-p \delta_{ij} + (v+v_t)(\frac{\partial{u_i}}{\partial x_j} + \frac{\partial{u_j}}{\partial x_i})]
\end{align}
where $U = (u_x, u_y)$ is the velocity field and $p$ the pressure, the unknown quantities to be determined. $\nu$ is the fluid viscosity considered as a constant, and $\nu_t$ is the so-called eddy viscosity.
$\nu_t$ can be determined using the widely-adopted Spalart-Allmaras equation \cite{spalart1992one}.  
 RANs equations of four partial differential equations in a two-dimensional space is obtained by integrating the Spalart-Allmarasa equation. 
 To solve this system, the Semi-Implicit Method for Pressure-Linked Equations (SIMPLE) algorithm is commonly employed (REFERENCE), operating under the assumption of incompressible fluid behavior. 
\textcolor{red}{tu ne parles pas des conditions aux limites ?}
\subsubsection{Machine Learning Scenario}
In the above context of airfoil flow problems, our objective is to construct a model able to predict fluid flow (velocity and pressure) around an airfoil based from its shape (and an associated mesh) and the two flow parameters, Angle of Attack (AoA) and Mach number (Mach), describing the specificities of the physical system. 
\\
To achieve this, we will train our GNN model using a dataset generated by a numerical CFD solver OpenFOAM, encompassing a variety of triplets (airfoil shapes, AoA, Mach).
To evaluate the performance of the proposed model, we will apply it to a series of flow problems with airfoil shapes that were never seen during training, and for various diverse physical parameters. This will allow us to assess the ability of the learned model to generalize to complex physical systems.    

==> Method.tex <==
\section{Method}
Real-world applications involve studying various airfoil shapes to optimize aircraft design for maximum energy capture and efficiency. It is crucial for machine learning models to maintain high performance for airfoil shapes not seen during the training phase or those that significantly differ from the training set (out-of-distribution -- OoD). Traditional supervised learning algorithms struggle with this, as they focus on learning from the available dataset without understanding the underlying PDE constraints of the physical system. As a result, predictions for airfoil shapes that differ from the training set may be worse than before.
\textcolor{red}{je propose quelque chose comme
It is known (il faudrait 1 ou 2 reférences) that a standard supervised learning approaches generalize well on samples that are interpolated from the training set, but perform much worse for extrapolated samples, i.e., OoD samples.}

\textcolor{red}{\bf En fait, il me semble que tout ce qui suit et la Section 4.1 devraient aller dans la Section 2, car d'une part elle n'est pas de toi, et d'autre part elle n'a rien de spéficifique  la CFD. La Section 2 serait alors plutôt "ML background" et ne parlerait pas du tout de CFD, et la partie 3 serait CFD Background, donnerait le ML scenario, et concluerait sur la nécessité d'utiliser du Meta Learning présenté en Section 2. Note que tu pourrais aussi inverser, et présenter d'abord le contexte CFD puis le Meta-Learning.\\
Après plus de réflexion, il faudrait en fait sans doute fusionner les sections 2 et 4.1 et les sections 3 et 4.2.
Mais on n'a pas le temps, donc on va laisser comme ça et juste aplanir les angles.}

Transfer learning has been proposed to improve the predictive accuracy of ML models, in particular regarding OoD points. 
Transfer learning can be simply employed by fine-tuning a pre-trained model on a small dataset of pairwise data from the OoD airfoil. Through a few steps of gradient descent optimization on this new dataset, we can potentially enhance the model performance on the OoD airfoil. This approach has low computational cost on training process and help alleviate overfitting concerns, as the pre-trained model serves as an initialization for the fine-tuning process. However, transfer learning may be less effective when limited data is available for the new task. This has been observed in studies of fine-tuning language models for text classification \cite{UniversalLanguage}, where the performance of the fine-tuned model was found to be significantly better than a model trained from scratch but was less effective when the dataset contained fewer than 100 examples. As a result, collecting data for fine-tuning a model on OoD airfoils can be resource-intensive, requiring running numerical simulations hundreds of times to generate new problem instances for each airfoil. This can be burdensome, especially when the model needs to be fine-tuned for multiple OoD airfoils.

To address this issue, we propose using meta-learning to train a meta-learner capable of adapting to new tasks or domains using fewer data points. 
Meta-learning, or learning to learn, involves training a model on a (meta-)distribution of tasks from the same meta-distribution such that it can quickly adapt to new tasks by leveraging its past experience. In the following section, we will discuss how meta-learning can be applied to improve the performance of a data-based approach on OoD airfoils.

\subsection{Model-Agnostic Meta-Learning Algorithms} 
Meta-learning provides a way to learn meta-knowledge over various tasks and to use this knowledge to learn new tasks using as few as possible task-specific data.  The model-agnostic meta-learning \cite{finn2017maml} (MAML) algorithm learns some initial parameters of a NN model that enable quick adaptation (fine-tuning) to new tasks with small amounts of data.  
\subsubsection{Problem Set-Up} A Meta-Learning dataset consists of a set of various tasks $\{\mathcal{T}_i, i=1,\ldots,N \}$. Each task ${\cal T}_i = \{\mathcal D_i, 
\mathcal L_i\}$ is made of a dataset $\mathcal D_i$ expressed as $\{(x_1^i, y_1^i), \ldots, (x_k^i, y_k^i) \}$ sampled from a distribution $p(\mathcal{T}_i)$, and a loss function $\mathcal{L}_i$ to be minimized. Each dataset $\mathcal{D}_i$ is split into a training and a test set: $\mathcal{D}_i = (\mathcal{D}_i^{tr},  \mathcal{D}_i^{test})$. Formally, the meta-training set is: $\mathcal{D}_{meta}^{tr} = \{(\mathcal{D}_i^{tr},  \mathcal{D}_i^{test})\}_i^{N}$. The meta learning model should be trained over different tasks $\{\mathcal{T}_i\}$, such that the trained model can quickly adapt to new tasks using only a small number of examples.
Formally, the optimal parameters of a meta-learner is: $$\theta_0 = \arg \min_\theta \sum_i \mathcal{L}_i(\mathcal{D}_i, \theta) $$

\subsubsection{Meta-Training} During Meta Training, some meta-knowledge $\theta_0$ is learned from $\mathcal{D}_{meta}^{tr}$. The meta-knowledge $\theta_0$ are trained to serve as a prior for the subsequent meta-test learning tasks.
Task-specific parameters $\theta_i$ are then computed based on $\mathcal{D}_i^{tr}$ and the meta-knowledge $\theta_0$. The MAML algorithm mentioned that one successful usage of prior knowledge is from fine-tuning where the pre-trained model $f_{\theta_0}$ from a similar task is considered as initialization, and used to train a new model using a few steps of gradient descent. Based on fine-tuning, MAML aims to find a partial model with parameters $\theta_i$, which can be easily fine-tuned for all tasks, even with small amounts of data. During meta training time, for each training task $\mathcal{T}_i$, the fine-tuning process is used to obtain the task-specific parameters $\theta_i$ and evaluate the task-specific model $f_{\theta_i}$ by samples from the test set $D_i^{test}$. The optimization target in this case is: 
\begin{equation}
    \theta_0 = \min_{\theta_0} \sum_{\mathcal{T}_i} \mathcal{L}_i (D_i ^{test}, \theta_i)
\end{equation}
$\theta_i$ is obtained by fine-tuning $w$ on $D_i^{tr}$: If N steps of gradient descent is applied, $\theta_i$ is expressed as:
\begin{equation}
\min\limits_{w} \sum\limits_{\mathcal{T}_i} \mathcal{L}_{\mathcal{T}_i}(f_{\theta_i^N}) = \min\limits_{w} \sum\limits_{\mathcal{T}_i} \mathcal{L}_{\mathcal{T}_i}(f_{\theta_i^{N-1} - \alpha \nabla_{\theta} L_{\mathcal{T}_i}(f(\theta_i^{N-1}))})\ 
\end{equation}

\subsubsection{Meta-Test} During Meta Test, given a new meta-test task $\mathcal{T} = \{(\mathcal{D}^{tr}, \mathcal{D}^{test}), \mathcal{L}\}$ sampled from the same meta-distribution as the training tasks $\mathcal{T}_1,\ldots,{\cal T}_N$, the task-specific parameters $\theta$ for the new task $\cal T$ is updated using the same fine-tuning method in the training process. The performance of the whole meta-learning algorithm is then evaluated on the test set $\mathcal{D}^{test}$ (and possibly for several different new meta-test tasks $\cal T$).

\subsubsection{MAML++} In fact, the update of the meta-parameters $\theta_0$ requires second-order derivatives. As a result, the bi-level optimization problem introduces instabilities when training the meta-learner. In order to mitigate these instabilities, \cite{maml++} proposed a multi-step loss optimization method (MSL). Instead of minimizing only the loss from the last step, the idea is to minimize the weighted sum of the losses at every updating step j, where the weights $w_j$ are pre-defined by users.
%: \Marc{d'où sortent les poids $w_j$ ???}
\begin{equation}
    \mathcal{L}_{meta} = \sum\limits_{\mathcal{T}_i} \sum_{j=1}^{N} w_j\mathcal{L}_{\mathcal{T}_i}(f_{\theta_i^j})
\end{equation}
In the following work, we will use the improved version MAML++ to train the meta-learner for the airfoil flow problems. 

\subsection{MAML for airfoil flow problems}
We formulate the airflow problem over various airfoils as a meta-learning problem (see Figure \ref{fig:diagram}), where each set of examples defined on a single airfoil shape is treated as a separate task. MAML++ is used to learn an incomplete model $f_{\theta_0}$, to be fine-tuned with a few steps of gradient descent, for any task, both from the meta-training set and the meta-test set. 
\begin{algorithm}
    \caption{Model-Agnostic Meta-learning Algorithm for Airfoil Flow}
    \label{alg:MAML}
        \begin{algorithmic}[1] 
        \Require Sample a set of airfoil shapes $\{\mathcal{A}_1, ..., \mathcal{A}_n \}$ from the shape distribution.
        \State Set learning rate parameters $\eta_1$, $\eta_2$
        \State Initialize the meta parameters $\theta_0$
        
        \For{every training airfoil $\mathcal{A}_i$ }
            \State Sample disjoint dataset $(D_i^{tr}, D_i^{test})$ from $\mathcal{A}_i$ by changing the two physical parameters AoA and Mach. 
            \State Evaluating gradient descent on $\theta$ with $D_i^{tr}$
            \State Compute adapted parameters:
            $\theta_i = \theta_0 - \eta_1 \nabla_{\theta_0} \mathcal{L} (D_i^{tr}, \theta_0)$
        \EndFor
        \State Update the meta-parameters $\theta_0 = \theta_0 - \eta_2 \nabla_{\theta_0} \sum_{\mathcal{T}_i} \mathcal{L}_i(\theta_i, D_i^{test})$ 
        \end{algorithmic}
\end{algorithm} 

\begin{figure}
    \centering
    \includegraphics[scale=0.45]{figures/diagram_MAML.png}
    \caption{Caption}
    \label{fig:diagram}
\end{figure}

%Based on these operators, it is straightforward to define a Graph U-Net model for PDE simulation. 

==> related_work.tex <==
\section{Related Work}
\subsubsection{Machine Learning for PDEs}
Machine learning algorithms have recently gained considerable attention for solving PDEs. 
Several works have proposed data-driven methods, making full use of labeled data accumulated by numerical solvers. The objective is to create a model capable of solving a family of PDEs of the same type. The inputs of the model are the physical quantities that define a specific instance of te target PDE, and the geometrical definition of the domain of interest where this PDE is defined. The 'labels' are the corresponding numerical solutions of the PDE. These methods learn a mapping from the physical and geometrical inputs to the corresponding solutions. 
Early works in 2D  \cite{shan2017study,Bhatnagar_2019,tompson2017accelerating,thuerey2020deep} considered the problem as an image-to-image problem and applied Convolutional Neural Networks (CNNs) in a straigtforward manner. 
%For instance, \cite{Bhatnagar_2019} employs the U-Net model \cite{unet} to address Reynolds Averaged Navier-Stokes (RANS) flow problems on airfoil shapes. The generated data on the unstructured mesh is first projected on structured grids as images before training. In comparison to traditional methods, CNN models can indeed reduce the overall computation time required to find solutions for new instances. 
However, such CNN approach only applies for image-like data. These researches either use structured meshes to discretize the physical domain, directly producing image-like data, or apply interpolation to convert mesh data into structured grids. As a result, they could not handle well problems with complex geometry. 
\\
In recent years, many attempts have been made to construct GNN models to cope with mesh data.  
\cite{kashefi2021point} discusses fluid flow field problems on different irregular geometries, considering CFD data as a set of points (called point clouds) and applying the PointNet\cite{qi2017pointnet} architecture specially designed for such a data type; \cite{pfaff2020learning} proposes a framework for learning mesh-based simulation problems with graph neural networks.
Both these data-driven approaches are extremely efficient compared with numerical solvers in terms of computational cost, however, they suffer from out-of-distribution generalization issues, as the underlying physical constraints are not included. 
\\
On the other hand, some works \cite{Berg_2018,raissi2018deep,raissi2019physics} based on unsupervised learning aim to design mesh-free methods, e.g., in the case of high dimensions or complex geometry. 
The basic idea of such methods is to put the physics in the loss during training. The inputs of the NN are the coordinates of some points in the domain, and the output is the solution $u$ of the PDE at hand. At inference time, the network directly predicts the value $u(x)$ when given $x$ as input. However, these unsupervised learning methods solve one problem each time (e.g., re-training is necessary when the boundary conditions change), and  require much more CPU time than data-based approaches, sometimes they are even slower than numerical solvers. 

\subsubsection{Meta-Learning} 
Meta-learning \cite{hospedales2021meta}, aka  "learning to learn", has emerged as a promising approach for training models that efficiently adapt to new tasks outside the ones used during training. In the context of multi-task learning, whereas standard machine learning algorithms are concerned with solving one single task, meta-learning involves learning, over several different tasks, some incomplete model that is able to learn a specialized models for all the tasks in the training set from only a few data points for each task. This incomplete model is then able to also learn new tasks with only a few data points. 
\\
Nowadays, there has been a growing trend in applying meta-learning algorithms to the approximation of PDEs \cite{qin2022meta,huang2022meta,chen2022meta}. These approaches often integrate optimization-based meta-learning algorithms \cite{finn2017maml,reptile}  with unsupervised learning methods for PDEs, such as physics-informed neural networks \cite{raissi2019physics} (PINNs). Researchers consider related parametric PDEs  as a set of related but distinct tasks and employ meta-learning principles to learn an initial model with strong generalization capabilities for these PDEs, thereby reducing the number of iterations required to adapt to a new PDE task. Such works partially reduce the computational cost for PINNs when a large number of PDEs with different parameters are to be solved, but are nevertheless still much less efficient than data-based approaches. 


